Scalable Sampling for High Utility Patterns

Discovering valuable insights from data through meaningful associations is a crucial task. However, it becomes challenging when trying to identify representative patterns in quantitative databases, especially with large datasets, as enumeration-based strategies struggle due to the vast search space involved. To tackle this challenge, output space sampling methods have emerged as a promising solution thanks to its ability to discover valuable patterns with reduced computational overhead. However, existing sampling methods often encounter limitations when dealing with large quantitative database, resulting in scalability-related challenges. In this work, we propose a novel high utility pattern sampling algorithm and its on-disk version both designed for large quantitative databases based on two original theorems. Our approach ensures both the interactivity required for user-centered methods and strong statistical guarantees through random sampling. Thanks to our method, users can instantly discover relevant and representative utility pattern, facilitating efficient exploration of the database within seconds. To demonstrate the interest of our approach, we present a compelling use case involving archaeological knowledge graph sub-profiles discovery. Experiments on semantic and none-semantic quantitative databases show that our approach outperforms the state-of-the art methods.

==> tex/Discussion.tex <==
To address in this section: ego-graphs, triangles, ... for social network interactions

\paragraph{Dense neighborhood ego-graph sampling}


\paragraph{Triangle sampling in social network}


\paragraph{Connected sub-network discovery in social network}

To be completed ...

~~\\

* T. Weng, X. Zhou, Y. Fang, K. -L. Tan and K. Li, "Finding Top-k Important Edges on Bipartite Graphs: Ego-betweenness Centrality-based Approaches," 2023 IEEE 39th International Conference on Data Engineering (ICDE), Anaheim, CA, USA, 2023, pp. 2415-2428, doi: 10.1109/ICDE55515.2023.00186.

~\\

* Liang Qu, Ningzhi Tang, Ruiqi Zheng, Quoc Viet Hung Nguyen, Zi Huang, Yuhui Shi, and Hongzhi Yin. 2023. Semi-decentralized Federated Ego Graph Learning for Recommendation. In Proceedings of the ACM Web Conference 2023 (WWW '23). Association for Computing Machinery, New York, NY, USA, 339–348. 


~\\

* J. Yang, Z. Huang, S. Quan, Z. Qi and Y. Zhang, "SAC-COT: Sample Consensus by Sampling Compatibility Triangles in Graphs for 3-D Point Cloud Registration," in IEEE Transactions on Geoscience and Remote Sensing, vol. 60, pp. 1-15, 2022, Art no. 5700115, doi: 10.1109/TGRS.2021.3058552.


~\\



* Counting and Sampling Triangles from a Graph Stream: A. Pavan†, Kanat Tangwongsan, Srikanta Tirthapura, Kun-Lung Wu, http://www.vldb.org/pvldb/vol6/p1870-aduri.pdf




~\\


* B. Wu, K. Yi and Z. Li, "Counting Triangles in Large Graphs by Random Sampling," in IEEE Transactions on Knowledge and Data Engineering, vol. 28, no. 8, pp. 2013-2026, 1 Aug. 2016, doi: 10.1109/TKDE.2016.2556663.

==> tex/Qualitative-experiments.tex <==
%!TEX root = ../QPlus.tex

In this section, we study the representativeness of the sampled patterns and check if the patterns drawn by \myalgo follow the same distribution that those drawn by \HAISampler in high average utility patterns sampling. Let the maximum length constraint be $\maxLen=10$ and the number of patterns to draw be $1,000$. We consider the following databases for evaluation:  \retail, \bmsDeux, and \chainstoreFIM. Figure \ref{fig:comparison_quality} gives the distribution of the average utility according the pattern lengths. 




\begin{figure}[htp!]
	\centering
	
	\includegraphics[width=.23 \textwidth, keepaspectratio]{img/retail_equiv.eps}
	\includegraphics[width=.23 \textwidth, keepaspectratio]{img/BMS2_equiv.eps}
	%\includegraphics[width=.23 \textwidth, keepaspectratio]{img/kosarak_equiv.eps}
	
	\includegraphics[width=.23 \textwidth, keepaspectratio]{img/chainstoreFIM_equiv.eps}
	\includegraphics[width=.23 \textwidth, keepaspectratio]{img/USCensus_equiv.eps}
	
	\caption{Comparing the distribution of 1,000 drawn patterns by \myalgo and \HAISampler }
	\label{fig:comparison_quality}
\end{figure}

%
%Let us now examine whether we have the same distribution as \HAISampler. Figure \ref{fig:comparison_quality} shows the distribution of the sampled patterns according to their lengths. 
Focusing on \myalgo on one hand, we can see that, the drawn patterns have high average utilities with different lengths. Interestingly, the most sampled patterns have very high utility values. 
On the other hand, as we can see that, we have approximately the same distribution in all of the considered quantitative databases which implies that \myalgo and \HAISampler follow the same distribution. Hence, we can conclude that our jumping based on dichotomous random search, Property \ref{prop:dichotomous_random_search}, sounds good.



